Sign Language Translation from Instructional Videos

The advances in automatic sign language translation (SLT) to spoken languages have been mostly benchmarked with datasets of limited size and restricted domains. Our work advances the state of the art by providing the first baseline results on How2Sign, a large and broad dataset. We train a Transformer over I3D video features, using the reduced BLEU as a reference metric for validation, instead of the widely used BLEU score. We report a result of 8.03 on the BLEU score, and publish the first open-source implementation of its kind to promote further advances.

==> Tables/ablation_inputs.tex <==
\begin{table*}[t]
\begin{tabular}{lccllclllclll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{ID}} & \multicolumn{4}{c}{\textbf{Changes}}                                                                                                                                & \multicolumn{4}{c}{\textbf{Val}}                   & \multicolumn{4}{c}{\textbf{Test}}                  \\
\multicolumn{1}{c}{}                    & baseline             & vocab size           & \begin{tabular}[c]{@{}l@{}}text\\ preprocessing\end{tabular} & \begin{tabular}[c]{@{}l@{}}param\\ transf\end{tabular} & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF \\ \hline
1                                       &                      &                      &                                                              &                                                        &                           &       &        &       &                           &       &        &       \\
2                                       &                      &                      &                                                              &                                                        &                           &       &        &       &                           &       &        &       \\
3                                       &                      &                      &                                                              &                                                        &                           &       &        &       &                           &       &        &       \\
4                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                              &                                                        & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\
5                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                              &                                                        & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\ \hline
\end{tabular}
\caption{Results for i3d finetuned for How2Sign.}
\label{tab:i3d_ft}
\end{table*}

\begin{table*}[t]
\begin{tabular}{lcclllclllclll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{ID}} & \multicolumn{5}{c}{\textbf{Changes}}                                                                                                                                                                                                   & \multicolumn{4}{c}{\textbf{Val}}                   & \multicolumn{4}{c}{\textbf{Test}}                  \\
\multicolumn{1}{c}{}                    & baseline             & vocab size           & \begin{tabular}[c]{@{}l@{}}text \\ preprocessing\end{tabular} & \begin{tabular}[c]{@{}l@{}}data \\ augm\end{tabular} & \begin{tabular}[c]{@{}l@{}}parameters \\ transformer\end{tabular} & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF \\ \hline
1                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
2                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
3                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
4                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                               &                                                      &                                                                   & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\
5                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                               &                                                      &                                                                   & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\ \hline
\end{tabular}
\caption{Results for OpenPose provided by the authors.}
\label{tab:op}
\end{table*}

\begin{table*}[t]
\begin{tabular}{lcclllclllclll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{ID}} & \multicolumn{5}{c}{\textbf{Changes}}                                                                                                                                                                                                   & \multicolumn{4}{c}{\textbf{Val}}                   & \multicolumn{4}{c}{\textbf{Test}}                  \\
\multicolumn{1}{c}{}                    & baseline             & vocab size           & \begin{tabular}[c]{@{}l@{}}text \\ preprocessing\end{tabular} & \begin{tabular}[c]{@{}l@{}}data \\ augm\end{tabular} & \begin{tabular}[c]{@{}l@{}}parameters \\ transformer\end{tabular} & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF & \multicolumn{1}{l}{sBLEU} & rBLEU & chrf-F & rCHRF \\ \hline
1                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
2                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
3                                       &                      &                      &                                                               &                                                      &                                                                   &                           &       &        &       &                           &       &        &       \\
4                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                               &                                                      &                                                                   & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\
5                                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                                               &                                                      &                                                                   & \multicolumn{1}{l}{}      &       &        &       & \multicolumn{1}{l}{}      &       &        &       \\ \hline
\end{tabular}
\caption{Results for MediaPipe.}
\label{tab:mp}
\end{table*}

